Positive Rate Binary Interactive Error Correcting Codes Resilient to $>\frac12$ Adversarial Erasures

An interactive error correcting code ($\mathsf{iECC}$) is an interactive protocol with the guarantee that the receiver can correctly determine the sender's message, even in the presence of noise. This generalizes the concept of an error correcting code ($\mathsf{ECC}$), which is a non-interactive $\mathsf{iECC}$ that is known to have erasure resilience capped at $\frac12$. The work of \cite{GuptaTZ21} constructed the first $\mathsf{iECC}$ resilient to $> \frac12$ adversarial erasures. However, their $\mathsf{iECC}$ has communication complexity quadratic in the message size. In our work, we construct the first positive rate $\mathsf{iECC}$ resilient to $> \frac12$ adversarial erasures. For any $\epsilon > 0$, our $\mathsf{iECC}$ is resilient to $\frac6{11} - \epsilon$ adversarial erasures and has size $O_\epsilon(n)$.

==> 3.5/3.5.tex <==
\section{$3/5$ Protocol}

\input{3.5/overview}
\input{3.5/protocol}
\input{3.5/analysis}

==> 3.5/analysis-correctness.tex <==
\subsubsection{Correctness Lemmas}

\begin{lemma}
    If Bob transitions to Phase 2 at the beginning of some block, Alice must have $\ind = \emptyset$, $\cnt = -1$, $\sent = \true$, and $\rec = \false$ at the start of the block.
    
    In particular, at any point in the protocol after Bob has entered Phase 2, if Alice's true input is $x = \hat{x}_b$ and she is in Stage 1, her state must be an element of $\Sigma_b$. If she is in Stage 2 with bit $\beta$, $\beta$ must be an element of $\Sigma_b$.
\end{lemma}

\begin{proof}
    Recall that Bob only sends $\bar{1}$ in Phase 1. If Alice has $\cnt = -1, \sent = \true$ when she receives a $\bar{1}$ from Bob, she can only increment $\cnt$ to $0$ and set $\sent = \false$. She does not update $\ind$, so $\ind = \emptyset$ still. On the other hand, if Alice ever has $\cnt = 0, \sent = \false$, she doesn't change either of these variables or $\ind$ upon receiving a $\bar{1}$. Thus, she always either has $\ind = \emptyset$ while Bob is in Phase 1. Then, at the beginning of the block when Bob transitions to Phase 2, Alice resets $\cnt = -1$, $\sent = \true$, $\rec = \false$. 
\end{proof}

\begin{lemma}
    At any point in the protocol after Bob enters Phase 2 and before he has set $\hat{x}$, it holds that:
    \begin{enumerate}[label={(\roman*)}]
        % \item Alice's value of $\ind$ is either a prefix of $i||1$, or is a prefix of $i||1$ with a $0$ appended to the end. In the latter case, her value of $\ind$ remains unchanged until Bob sets $\hat{x}$.
        \item For any $(\ind_0, \cnt_0, \sent_0, \rec_0) \in \Sigma_0$ and $(\ind_1, \cnt_1, \sent_1, \rec_1) \in \Sigma_1$, it holds that $\big| |\ind_0| - |\ind_1| \big| \le 1$. Also, if $\ind_0 = \ind_1$, then $\ind_0 = \ind_1$ is a prefix of $i||1$.
        \item For any chunk for which $j \not\in \IGNORE$, $S_0 \cap S_1 = \emptyset$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    Assume for the sake of contradiction there exists an execution of the protocol in which at some point one of the conditions (i),(ii) is violated. Let $V$ be the first chunk after which this is true, and let $W \le V$ be the last chunk whose number $j \not\in \IGNORE$ in which Alice's message to Bob was $< (\frac34 - \frac?? \epsilon)$-erased, so that Bob list-decoded Alice's message to two possibilities $m_0$ and $m_1$. Since $m_0 \in S_0$ and $m_1 \in S_1$ (otherwise Bob would've set $\hat{x}$) and (i),(ii) hold at the start of chunk $W$, it holds that $m_0 \not= m_1$, and property (i) holds for $m_0$ and $m_1$ if $m_b = \ECC \left( \ECC'(\hat{x}_b) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind_b, \cnt_b, \sent_b, \rec_b \right)$.
    
    We show that conditions (i),(ii) must still hold after chunk $V$ via casework on $m_0, m_1$. Recall that $S_b$ is determined by the set $\Sigma_b$, and since for any chunk $j \not\in \IGNORE$ it holds that $\ECC'(\hat{x}_0) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right] \not= \ECC'(\hat{x}_1) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right]$, it suffices for condition (ii) to show that the same bit $\beta$ cannot belong to both $\Sigma_0$ and $\Sigma_1$ simultaneously.
    
    We remark that Alice only alters $\ind$ or advances to Stage 2 inbetween blocks, so if she sent a value of $\ind$ during a block, all her future messages in that block must also contain the same value $\ind$. In particular, (i),(ii) hold trivially whenever $V$ is in the same block as $W$. We therefore only consider the case where $V$ is in a later block.
    
    % Assume for the sake of contradiction there exists an execution of the protocol in which at some point $S_0 \cap S_1 \not= \emptyset$. Let $V$ be the first chunk such that $\no(V+1) \not\in \IGNORE$ \rnote{notation??} after which this is true, and let $W \le V$ be the last chunk with $\no(W) \not\in \IGNORE$ in which Alice's message to Bob was $< (\frac34 - \frac??\epsilon)$-erased, so that Bob list-decoded Alice's message to two possibilities $m_0$ and $m_1$. Since $S_0 \cap S_1 = \emptyset$ right before chunk $W$ and $m_0 \in S_0, m_1 \in S_1$, it follows that $m_0 \not= m_1$. 
    
    % Recall that whenever $j \not\in \IGNORE$, $\ECC'(\hat{x}_0) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right] \not= \ECC'(\hat{x}_1) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right]$. Therefore, since $\hat{x}_0 \not= \hat{x}_1$ (otherwise $\hat{x}$ would have already been set), $S_0$ and $S_1$ cannot share any elements of the form $\ECC(s, \ind, \cnt, \sent, \rec)$. It suffices to show that $S_0$ and $S_1$ after chunk $V$ do not share any elements of the form $\beta^{4P}$, or equivalently $\Sigma_0$ and $\Sigma_1$ do not share any element $\beta$.
    
    \begin{caseofp}
    \begin{mdframed}[topline=false,rightline=false,bottomline=false]
    \casep{$m_b = \left\{ \ECC \left( \ECC'(\hat{x}_b) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind_b, \cnt_b, \sent_b, \rec_b \right) \right\}$ for $b = 0, 1$.}{
        \begin{subcaseofp}
        \subcasep{$\ind_0 \not= \ind_1$. Bob has sent all $\bar{1}$'s or all $\bar{0}$'s for the entirety of the block containing chunk $W$, and $\bar{0}$'s after.}{
            If Bob has only sent $\bar{1}$'s in the block containing $W$, then since Alice must've started the block with $\cnt = -1$ and $\sent = \true$, her new values of $\cnt, \sent$ must be either $(-1, \true)$ or $(0, \false)$. Either way, she does not advance to Stage 2 or modify $\ind$ at the end of the block.
            
            This means that at the start of a block before or including $V$, and after or including $W$, Bob has sent only $\bar{0}$'s while $\Sigma_b = \{ (\ind_b, \cnt_b = -1, \sent_b = \true, \rec_b = \false) \}$. Alice cannot modify $\ind$ in this state, so (i) holds after chunk $V$ still. If the Alice corresponding to $\hat{x}_b$ receives a $\bar{0}$ and advances to Stage 2, she must advance with the bit $|\ind_b|~\text{mod}~2$, which is different for $b = 0,1$ since $|\ind_0| = |\ind_1| \pm 1$. 
        }
        \subcasep{$\ind_0 = \ind_1$, and w.l.o.g. $\cnt_0 = -1$, $\cnt_1 = 0$. Bob sends $\bar{0}$ for the rest of the block containing $W$, then $\bar{1}$ thereafter. %In the block containing $W$, Bob had sent $\bar{1}$ until the first time he saw $\cnt_0 = -1, \cnt_1 = 0$, then had sent $\bar{0}$ for the rest of the block, and $\bar{1}$ thereafter.
        }{
            The Alice corresponding to $\cnt = -1$ may or may not receive a $\bar{0}$ in that block containing $W$. If she doesn't, she begins the next block still in Stage 1, with the same value of $\ind_0$. If she does, she advances at the beginning of the next block to Stage 2 with the bit $\beta_0 = (|\ind_0|~\text{mod}~2)$. Recall that receiving a $\bar{1}$ while $\cnt = -1$ can never cause Alice to alter $\ind_0$ or advance to Stage 2, so these are the only two possibilities.
            
            The Alice corresponding to $\cnt = 0$ has only received $\bar{0}$, if anything, within the same block as $W$. Then, at the end of the block, either she makes no update or she appends $0$ to $\ind_1$. Receiving $\bar{1}$ in future blocks does not cause her to alter $\ind_1$ further.
            
            To summarize, after chunk $V$, Alice 0 is either still in Stage 1 with the same value of $\ind_0$, or is in Stage 2. Alice 1 either has $\ind_1 = \ind_0$ still, or $\ind_1 = \ind_0 || 0$. Properties (i),(ii) still hold.
        }
        \subcasep{$\ind_0 = \ind_1$, and w.l.o.g. $\cnt_0 = 0$, $\cnt_1 = 1$. Bob has sent $\bar{1}$ since.}{
            Note that the only way that $\cnt_0 = 0$ and $\cnt_1 = 1$ is if $i[|\ind_0| + 1] = 1$ (otherwise, when $\cnt_0 = \cnt_1 = 0$ Bob would've sent $\bar{0}$ for the rest of the block). 
            
            Consider the first chunk $W'$ in the same block as $W$ in which Bob $2$-decoded Alice's message in a chunk with $j \not\in \IGNORE$ for which $\ind_0 = \ind_1$ and $\cnt_0 = 0, \cnt_1 = 1$. In order to have gotten to this point, every time Bob previously 2-decoded Alice's message in a chunk with $j \not\in \IGNORE$, he must've seen $\cnt_0 = \cnt_1$. This means that the only time he ever sent $\bar{0}$ this block was after confirming both Alices had $\rec_0 = \rec_1 = \true$. \rnote{hmm wait there is an issue which is cnt0=cnt1=0 and rec0=false,rec1=true. then bob sends 0 which advances alice 0 but alice 1 stays. need a mechanism to tell if alice has already committed to appending.}
            
            Alice 0 can only receive $\bar{1}$ in the block containing $W$. Then, at the end of the block, she either appends $1$ to $\ind_0$ if she had incremented $\cnt_0$ to $1$ during the block, or she does nothing to $\ind_0$ (note that it's not possible for her to append $0$ to $\ind_0$ since she's only received $\bar{1}$).
        }
        \subcasep{$\ind_0 = \ind_1$, $\cnt_0 = \cnt_1 < i[|\ind_0| + 1]$, and $\rec_0 = \rec_1 = \false$. Bob has sent $\bar{1}$ since.}{
            
        }
        \subcasep{$\ind_0 = \ind_1$, $\cnt_0 = \cnt_1 < i[|\ind_0| + 1]$, and $\rec_0 \vee \rec_1 = \true$. Bob has sent $\bar{0}$ for the rest of the group and $\bar{1}$ thereafter.}{
            
        }
        \subcasep{$\ind_0 = \ind_1$, $\cnt_0 = \cnt_1 = i[|\ind_0| + 1]$. Bob has sent $\bar{0}$ for the rest of the block and $\bar{1}$'s thereafter.}{
            
        }
        \end{subcaseofp}
    }
    \casep{$m_b = \beta_b^{4P}$ and $m_{1-b} = \ECC \left( \ECC'(\hat{x}_{1-b}) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind_{1-b}, \cnt_{1-b}, \sent_{1-b}, \rec_{1-b} \right)$.}{
        \begin{subcaseofp}
        \subcasep{$|\ind_{1-b}| \equiv 1 - \beta_b \Mod{2}$. }{}
        \end{subcaseofp}
    }
    \end{mdframed}
    \end{caseofp}
\end{proof}


==> 3.5/analysis-error-resilience.tex <==
\subsubsection{Erasure Resilience}

==> 3.5/analysis.tex <==
\subsection{Analysis}

\input{3.5/analysis-correctness}
\input{3.5/analysis-error-resilience}


==> 3.5/overview.tex <==
\subsection{Protocol Overview}

==> 3.5/protocol.tex <==
\subsection{Formal Protocol} \label{sec:3/5-formal}

\protocol{Interactive Binary One Way Protocol Resilient to $\frac35 - \frac{?}{?} \epsilon$ Erasures}{3/5}{
    \setlength{\parindent}{1em}

    Let $n$ be the size of the message $x \in \{ 0, 1 \}^n$ that Alice wishes to convey to Bob. Without loss of generality, $n$ is a power of $2$. Let 
    \begin{align*}
        \E(x) : \{ 0, 1 \}^n \rightarrow \{ 0, 1 \}^M
    \end{align*}
    be an error correcting code as in \ref{thm:ECC} of relative distance $\frac12-\epsilon$.
    
    Furthermore, let
    \begin{align*}
        \ECC(s, \ind, \cnt, \sent, \rec) : \{ 0, 1 \}^{\log n} \times \{ 0, 1 \}^{\log n + 1} \times \{ -1, 0, 1 \} \times \{\true, \false \} \times \{ \true, \false \} \rightarrow \{ 0, 1 \}^{4P}
    \end{align*}
    be an error correcting code of relative distance $\frac12-\epsilon$ such that each codeword is also relative distance $\ge \frac12 - \epsilon$ from each of $0^{4P}, 1^{4P}$, as given in Theorem~\ref{thm:ECC}. Also, let $\bar{0}=0^P$ and $\bar{1}=1^P$. Our protocol consists of $\frac{M}{\epsilon \log n}$ blocks $C = \frac{M}{\epsilon^3 \log n}$ chunks, each of which consists of $\frac1\epsilon$ groups of $\frac1\epsilon$ chunks, each consisting of a $4P$ bit message from Alice followed by a $P$ bit message from Bob. We label each chunk with a number in $\left[ \frac{M}{\log n} \right]$: the $k$'th chunk is labeled with $k ~\text{mod}~ \frac{M}{\log n}$, where if $k \equiv 0 \Mod{\frac{M}{\log n}}$ it is labeled instead with $\frac{M}{\log n}$. Throughout the protocol, the parties will choose a response based on which case applies to their received message $m$; if multiple apply, they choose the first case on the list.
    
    \begin{center}
    {\bf \fbox{Alice}}
    \end{center}
        
    Alice's message will always be from the following set: $$\{ \ECC(s,\ind,\cnt,\sent,\rec) \}_{x,\ind,\cnt,\sent,\rec} \cup \{ 0^{4P}, 1^{4P} \}$$ which has relative distance $\ge \frac12 - \epsilon$. She tracks certain values explicitly, namely the \emph{stage} of the protocol she is in, and the following variables:
    \begin{itemize}
    \item 
        A variable $\ind \in \{ 0, 1 \}^{\le \log n + 1}$, initially set to the empty string $\emptyset$.
    \item 
        A variable $\cnt \in \{ -1, 0, 1 \}$, initially set to $-1$.
    \item 
        A bit $\sent \in \{\true,\false\}$ denoting whether she has received a $0$ from Bob after sending this particular value of $\ind$ (i.e. whether she has received \emph{confirmation} that $\ind$ was successfully sent to Bob) within this block. Initially $\sent$ is set to $\true$.
    \item 
        A bit $\rec \in \{\true,\false\}$ denoting whether she has \emph{received} a $1$ so far this block. $\rec$ is initially set to $\false$.
    \end{itemize}
        
    Alice acts differently according to which of three stages she is in. She begins in in Stage 1, where she appends to $\ind$. At some point, she advances to Stage 2, where she sends only a single bit $\beta$ for the rest of the protocol.
        
    \begin{enumerate}[align=left, leftmargin=*, label={\bf Stage \arabic*:}]
    
    \item 
        At the beginning of each block, she resets $\cnt \gets -1$ and $\sent \gets \true$. At the beginning of each group, she additionally resets $\rec \gets \false$.
        
        Every message, Alice sends $\ECC \left( \ct \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind, \cnt, \sent, \rec \right)$, where $j$ is the number of the current chunk.
        
        Before every message except for the first in each group, Alice updates $\ind, \cnt, \sent, \rec$ based on the most recent message $m \in \{ 0, 1, \perp \}^P$ received from Bob, as follows. Note that if $m$ is not entirely erased, then Alice can uniquely decode $m$ to one of $\bar{0}$ and $\bar{1}$.
        
        \begin{caseof}
            
            \case {All of the symbols in $m$ are $\perp$.}{
                Alice does no update.
            }
                
            \case {$m$ decodes uniquely to $\bar{1}$.}{
                Alice sets $\rec \gets \true$. If $\sent = \true$, she increments $\cnt$ and sets $\sent \gets \false$. 
                
                If $\cnt = 1$, she does no further updates for the rest of the block. At the end of the block, she appends $1$ to the end of $\ind$. If $|\ind| = \log n + 1$ and $\ind[\log n + 1] = 1$, she advances to Stage 2 with $\beta = x[\ind]$.
            }
                
            \case {$m$ decodes uniquely to $\bar{0}$, and $\rec = \true$ (i.e. she's already seen a $1$ this group).}{
                Alice sets $\sent \leftarrow \true$. 
            }
                
            \case {$m$ uniquely decodes to $\bar{0}$, and $\rec = \false$ (i.e. she has seen no messages this group and the first message received is a $\bar{0}$).}{
                If $\cnt = -1$, she advances to Stage 2 with $\beta = |\ind| ~\text{mod}~ 2$.
                
                If $\cnt = 0$, does no further updates for the rest of the block. At the beginning of the next block, she appends $0$ to the end of $\ind$.
            }
            
        \end{caseof}
            
    \item 
        When Alice reaches this stage, she has noted a bit $\beta$. She sends this for the rest of the protocol; all her messages from here on out are irreversibly $\beta^{4P}$. 
        
    \end{enumerate}
        
    \begin{center}
    {\bf \fbox{Bob}}
    \end{center}
    
        Bob holds a variable $\hat{x}$, initially set to $\emptyset$, representing his final output. It will either be set at the end of the protocol or sometime during the protocol if he unambiguously learns Alice's value of $x$. In either case, once set it is final, and at the end of the protocol, Bob outputs $\hat{x}$. We remark that once $\hat{x}$ is set, Bob may behave arbitrarily for the rest of the protocol: let us say that he simply sends $\bar{1}$ for each message thereafter and does no further updates to any of his internal variables.
        
        Bob tracks which phase he is in explicitly, and he holds certain values to help him perform consistency checks of 2-decoded Alice's messages with previous pairs:
        \begin{itemize}
            \item $\hat{x}_0$ and $\hat{x}_1$ storing two possible values of $x$ Alice holds.
            \item $\Sigma_0$ and $\Sigma_1$ storing all possible values of $(\ind, \cnt, \sent, \rec)$ that Alice may currently hold if she is still in Phase 1, or $\beta$ if she is in Phase 2, that are consistent with previous 2-decoded pairs of messages, corresponding to her holding the input $\hat{x}_0$ and $\hat{x}_1$ respectively.  Initially $\Sigma_0$ and $\Sigma_1$ are both initialized to $\{ (\ind = \emptyset, \cnt = -1, \sent = \true, \rec = \false) \}$.
            \item $S_0$ and $S_1$ storing all possible messages Alice could send next that are consistent with previous 2-decoded pairs of messages, corresponding to her holding the input $\hat{x}_0$ and $\hat{x}_1$ respectively. At any point, if the next message Alice sends is in a chunk numbered $j$, the set $S_b$ consists of all values $\ECC \left( \ECC'(\hat{x}_b) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind_b, \cnt_b, \sent_b, \rec_b \right)$ for $(\ind_b, \cnt_b, \sent_b, \rec_b) \in \Sigma_b$, along with the value $\beta_b^{4P}$ for any $\beta_b \in \{ 0, 1 \}$ in $\Sigma_b$. 
            \item A bit $\ans$, initially set to $\emptyset$, that will be set to the bit Bob expects to receive in Phase 4 from the Alice corresponding to $\hat{x}_1$.
        \end{itemize}
        
        Bob will set $\hat{x}_0$ and $\hat{x}_1$ in Phase 1. Starting in Phase 2, he updates $\Sigma_0, \Sigma_1$ every time he receives a message $m \in \{ 0, 1, \perp \}^{4P}$ from Alice in a chunk numbered $j \not\in \IGNORE$ where $m$ is $< (\frac34 - \frac?? \epsilon)$-erased, \emph{as well as} after each message he sends, as follows:
        
        \begin{itemize}
            \item If Bob does not set $\hat{x}$ in response to receiving a message $m$, then $m$ must be 2-decodable to $m_0, m_1$, where $m_0 \in S_0$ and $m_1 \in S_1$. For each $b \in \{ 0, 1 \}$, if $m_b = \ECC \left( \ECC'(\hat{x}_b) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind_b, \cnt_b, \sent_b, \rec_b \right)$ for some $\ind_b, \cnt_b, \sent_b, \rec_b$, he sets $\Sigma_b = \{ (\ind_b, \cnt_b, \sent_b, \rec_b) \}$. Otherwise, if $m_b = \beta_b^{4P}$ for some $\beta_b \in \{ 0, 1 \}$, he sets $\Sigma_b = \{ \beta_b \}$.
            \item Each time after Bob sends a message, he calculates for each $\sigma_b = (\ind_b, \cnt_b, \sent_b, \rec_b) \in \Sigma_b$ the $\le 2$ new states that Alice could have if she had or hadn't received his message, and puts these in the updated set $\Sigma_b$. (He does this adhering to starts of blocks and groups: if it is the start of a group, he sets the values of $\sent, \rec$ to $\true, \false$, and if it is the start of a block, he sets $\cnt$ to $-1$.) If Alice advances if she receives his message, he instead adds the value $\beta_b$ to $\Sigma_b$, where $\beta_b$ is the bit she'd advance with. Furthermore, for any $\sigma_b \in \{ 0, 1 \}$ in $\Sigma_b$, he puts $\sigma_b$ in the updated set $\Sigma_b$.
        \end{itemize}
        
        Each of Bob's messages throughout the protocol is either $\bar{0}$ or $\bar{1}$. Bob's next message is dependent on the phase he is currently in. He begins in Phase 1, and eventually moves to Phase 2. From there, he may transition straight to Phase 4, or first through Phase 3 before going to Phase 4. 
        
        \begin{enumerate}[align=left, leftmargin=*, label={\bf Phase \arabic*:}]
        \setcounter{enumi}{0}
        
        \item 
            In Phase 1, Bob sends $\bar{1}$ every message. Meanwhile, for each $k \in \bbN$, after the $\frac{kM}{\log n}$'th chunk, if there have been less than $\left( \frac34 - \frac?? \epsilon \right) \cdot \frac{MP}{\log n}$ erasures in Alice's messages in the past $\frac{M}{\log n}$ chunks, Bob finds at most two values of $x$ for which there exist $\{ (\ind_j, \cnt_j, \sent_j, \rec_j) \}_{j \in [\frac{M}{\log n}]}$ such that $\ECC \left( \ECC'(x) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind_j, \cnt_j, \sent_j, \rec_j \right)$ is compatible with the $j$'th message. \rnote{needs to be reworded} He sets $\hat{x}_0, \hat{x}_1$ to be these two values of $x$. Then, at the end of the block, Bob transitions to Phase 2. 
        
        \item 
            In Phase 2, Bob's goal is to append to Alice's value of $\ind$ so that it is equal to $i || 1 \in \{ 0, 1 \}^{\log n + 1}$, where $i$ is an index for which $\hat{x}_0[i] \not= \hat{x}_1[i]$. 
            
            Let $\IGNORE$ be the set of values $j \in \left[ \frac{M}{\log n} \right]$ for which $\ECC'(\hat{x}_0) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right] = \ECC'(\hat{x}_1) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right]$. 
            
            At the start of each group, Bob sends $\bar{1}$. For every other message in the group, Bob determines what he sends next based on the following cases for the message $m \in \{ 0, 1, \perp \}^{4P}$ he most recently received from Alice. In what follows, $j \in \left[ \frac{M}{\log n} \right]$ denotes the number of the current chunk.
            
            \begin{caseof}
            \case {$m$ has at least $\frac34 - \frac??\epsilon$ $\perp$'s or $j \in \IGNORE$.}{
                Bob repeats his last message.
            }
            \case {Bob $\leq 2$-decodes $m$ to $\{ m_0, m_1 \}$, and there exists $b \in \{ 0, 1 \}$ such that $m_0, m_1 \not\in S_b$.}{
                Bob sets $\hat{x}\gets\hat{x}_{1-b}$.
            }
            \end{caseof}
        
            In all remaining cases, Bob $2$-decodes $m$ to two messages $m_0 \in S_0$ and $m_1 \in S_1$. 
            
            \begin{caseof}
            \setcounter{casenum}{3}
            
            \case {One of the Alices has already advanced, that is, for some $b \in \{ 0, 1 \}$, $m_b \in \{ 0^{4P}, 1^{4P} \}$.}{
                Let $m_b = \beta_b^{4P}$, where $\beta_b \in \{ 0, 1 \}$. The other $m_{1-b}$ must be of the form $\ECC \left( \ECC'(\hat{x}_{1-b}) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind_{1-b}, \cnt_{1-b}, \sent_{1-b}, \rec_{1-b} \right)$.
                
                Bob sends $\bar{1}$ for the rest of the block. He sets $\ans \gets (\mathbbm{1}[b=0] + \beta_b ~\text{mod}~ 2)$. At the beginning of the next block, he transitions to Phase 3 if $|\ind_{1-b}| \equiv \beta_b \Mod{2}$, or Phase 4 if $|\ind_{1-b}| \equiv 1 - \beta_b \Mod{2}$.
            }
            \end{caseof} 
            
            For the rest of the cases, $m_b = \ECC \left( \ECC'(\hat{x}_b) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind_b, \cnt_b, \sent_b, \rec_b \right)$, and $\ECC'(\hat{x}_0) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right] \not= \ECC'(\hat{x}_1) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right]$
            
            \begin{caseof}
            \setcounter{casenum}{4}
            
            \case{$\ind_0 \not= \ind_1$.}{
                Bob sends $\bar{1}$ for the rest of the block. He sets $\ans \gets (|\ind_1| ~\text{mod}~ 2)$, and at the beginning of the next block transitions to Phase 4.
            }
            
            \case{$\ind_0 = \ind_1$, and $\cnt_b = -1$, $\cnt_{1-b} = 0$.}{
                Bob sends $\bar{0}$ for the rest of the block.
            }
            
            \case{$\ind_0 = \ind_1$, and $\cnt_b = 0$, $\cnt_{1-b} = 1$.}{
                Bob sends $\bar{1}$ for the rest of the block.
            }
            
            \case{$\ind_0 = \ind_1$, $\cnt_0 = \cnt_1 < i[|\ind_0| + 1]$, and $\rec_0 = \rec_1 = \false$.}{
                Bob sends $\bar{1}$.
            }
            
            \case{$\ind_0 = \ind_1$, $\cnt_0 = \cnt_1 < i[|\ind_0| + 1]$, and $\rec_0 \vee \rec_1 = \true$.}{
                Bob sends $\bar{0}$.
            }
            
            \case{$\ind_0 = \ind_1$, $\cnt_0 = \cnt_1 = i[|\ind_0| + 1]$}{
                Bob sends $\bar{0}$ for the rest of the block.
            }
            
            \end{caseof}
            
        \item 
            If Bob enters Phase 3, it is at the start of a block, and he decoded to two states $m_0, m_1$ in the last block, where $m_b = \beta_b^{4P}$ for some $\beta_b \in \{ 0, 1 \}$, and $m_{1-b} = \ECC \left( \ECC'(\hat{x}_{1-b}) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind_{1-b}, \cnt_{1-b}, \sent_{1-b}, \rec_{1-b} \right)$ such that $|\ind_{1-b}| \equiv \beta_b \Mod{2}$. 
            
            The first message of each block that Bob sends is a $\bar{1}$. For all other messages, he does the following based on the most recent message $m \in \{ 0, 1, \perp \}^{4P}$ he received from Alice.
            
            \begin{caseof}
            
            \case{$m$ has at least $\frac34 - \frac?? \epsilon$ $\perp$'s or $j \in \IGNORE$.}{
                Bob repeats his last message.
            }
            
            \case{Bob $\le 2$-decodes $m$ to $\{ m_0, m_1 \}$, and there exists $b \in \{ 0, 1 \}$ such that $m_0, m_1 \not\in S_b$.}{
                Bob sets $\hat{x} \gets \hat{x}_{1-b}$.
            }
            
            \end{caseof}
            
            In all remaining cases, Bob $2$-decodes $m$ to messages $m_b = \beta_b^{4P}$ and $m_{1-b} = \ECC \left( \ECC'(\hat{x}_{1-b}) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], \ind_{1-b}, \cnt_{1-b}, \sent_{1-b}, \rec_{1-b} \right)$. 
            
            \begin{caseof}
            \setcounter{casenum}{3}
            
            \case{$|\ind_{1-b}| \equiv 1 - \beta_b \mod{2}$.}{
                Bob sends $\bar{1}$ for the rest of the block, then at the beginning of the next block, he transitions to Phase 4.
            }
            
            \case{$\cnt_{1-b} = -1$.}{
                Bob sends $\bar{1}$.
            }
            
            \case{$\cnt_{1-b} = 0$.}{
                Bob sends $\bar{0}$.
            }
            
            \end{caseof}
            
        \item 
            When Bob enters Phase 4, it is at the start of a block, and $\ans$ has been set to a bit. He sends $\bar{0}$ for the rest of the protocol. At the end of the protocol, let $B$ be the most recent bit Bob has received from Alice. He sets $\hat{x} \gets \hat{x}_{\mathbbm{1}[B = \ans]}$
   
        \end{enumerate}
}

==> ECC.tex <==
\section{Error Correcting Codes}

\begin{lemma} \label{lem:ECC-well-spread}
    There exists a family of error correcting codes $\ECC = \{ \ECC_n : \{ 0, 1 \}^n \rightarrow \{ 0, 1 \}^{M(n)} \}_{n \in \bbN}$ with relative distance $\frac12 - \epsilon$ and $M = O_\epsilon(n)$ that satisfies that for all $x, y \in \{ 0, 1 \}^n$, 
    \[
        \left| \left\{ j \in [M/\log n] : \ECC(x) \left[ \frac{(j-1)M}{\log n} + 1 : \frac{jM}{\log n} \right] = \ECC(y) \left[ \frac{(j-1)M}{\log n} + 1 : \frac{jM}{\log n} \right] \right\} \right| \le \frac{\epsilon M}{\log n}.
    \]
\end{lemma}

\begin{proof}
    Note that this holds for a random code: for any two strings $x, y \in \{ 0, 1 \}^n$ the expected number of the $M/\log n$ strings that are equal is $2^{-\log n} \cdot M/\log n$ and the variance is $\approx 2^{-\log n} \cdot M/\log n$, so the probability that at least $\epsilon$ fraction of the $M/\log n$ strings are the same is at most $\approx 2e^{-\epsilon^2 n \log n \cdot M}$ by Chernoff. Union bounding over all $2^{2n}$ pairs of strings $x, y$, we get that the probability the above property holds is at least $\approx 1$.
\end{proof}

Let $\ECC$ be a family of error correcting codes $\{ \ECC_n : \{ 0, 1 \}^{\log n} \times \{ 0, 1 \}^{\le \log n} \rightarrow \{ 0, 1 \}^{P(n)}$ with relative distance $\frac12 - \epsilon$ and $P = O_\epsilon(\log n)$. 

\begin{lemma}
    Define $C : \{ 0, 1 \}^n \times (\{ 0, 1 \}^{\le \log n})^{M/\log n}$
    \[
        C(x; r_1, \dots, r_{M/\log n}) = \ECC \left( \ct\left[ 1 : \log n \right], r_1 \right) || \dots || \ECC \left( \ct\left[ M - \log n + 1 : M \right], r_{M/\log n} \right),
    \]
    where $\ECC$ is a family of error correcting codes $\{ \ECC_n : \{ 0, 1 \}^{\log n} \times \{ 0, 1 \}^{\le \log n} \rightarrow \{ 0, 1 \}^{P(n)}$ with relative distance $\frac12 - \epsilon$, and $\ct = \ECC'(x)$ where $\ECC' = \{ \ECC'_n : \{ 0, 1 \}^n \rightarrow \{ 0, 1 \}^N \}_{n \in \bbN}$ satisfies the properties listed in Lemmma~\ref{lem:ECC-well-spread}.
    
    Then for any $x \not= y \in \{ 0, 1 \}^n$ and any $(r_1, \dots, r_{M/\log n}), (s_1, \dots, s_{M/\log n}) \in (\{ 0, 1 \}^{\le n})^{M/\log n}$, it holds that 
    \[
        \Delta(C(x; r_1, \dots, r_{M/\log n}), C(y; s_1, \dots, s_{M/\log n})) \ge \left( \frac12 - \frac32 \epsilon \right) \cdot \frac{MP}{\log n}.
    \]
\end{lemma}

\begin{proof}
    On all but at most $\frac{\epsilon M}{\log n}$ of the intervals $\left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right]$, $\ECC'(x)$ and $\ECC'(y)$ are not identical. For each such interval $\left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right]$, 
    \[
        \Delta \left( 
            \ECC \left( \ECC'(x) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], r_j \right),
            \ECC \left( \ECC'(y) \left[ \frac{(j-1)M}{\log n} + 1, \frac{jM}{\log n} \right], s_j \right)
        \right)
        \ge \left( \frac12 - \epsilon \right) \cdot P,
    \]
    so that 
    \begin{align*}
        \Delta(C(x; r_1, \dots, r_{M/\log n}), C(y; s_1, \dots, s_{M/\log n}))
        \ge \frac{(1-\epsilon)M}{\log n} \cdot \left( \frac12 - \epsilon \right) \cdot P 
        \ge \left( \frac12 - \frac32 \epsilon \right) \cdot \frac{MP}{\log n}.
    \end{align*}
\end{proof}
